Measurement of electrons from semileptonic heavy-flavour hadron decays in pp collisions at $\sqrt{s}$= 7 TeV

The differential production cross section of electrons from semileptonic heavy-flavour hadron decays has been measured at mid-rapidity ($|y| < 0.5$) in proton-proton collisions at $\sqrt{s} = 7$ TeV with ALICE at the LHC. Electrons were measured in the transverse momentum range 0.5 $<p_{\rm T}<$ 8 GeV/$c$. Predictions from a fixed order perturbative QCD calculation with next-to-leading-log resummation agree with the data within the theoretical and experimental uncertainties.

==> normalization.tex <==
To calculate the \pt differential production cross section, the measured 
electron yield has to be normalised to the integrated luminosity or to the 
measured cross section of a chosen reference process. Here, the minimum bias 
condition itself is adopted as reference process.

The minimum bias cross section $\sigma_{\rm MB}$ has been obtained relative to the 
cross section $\sigma_{\rm VOAND}$~\cite{MBcrosssection,MBcrosssectionbis} of the 
coincidence between signals in the two VZERO detectors as measured in a 
van der Meer scan. The relative factor $\sigma_{\rm VOAND} / \sigma_{\rm MB}$ is equal 
to 0.873 and stable within 1\% over the analysed data sample. The value for
$\sigma_{\rm MB}$ is \mbox{71.4$\pm$0.7(stat)$\pm$7.1(syst)~mb}. With that the 
measured electron yields $N$ can be converted into a differential cross section:

\begin{equation}
\frac{1}{2\pi \pt} \frac{d^{2}\sigma}{d\pt dy} = 
\frac{\sigma_{\rm MB}}{N_{\rm MB}}\frac{1}{2\pi \pt} \frac{d^{2}N}{d\pt dy}
\end{equation}

The normalisation to an absolute cross section contains an additional 
source of systematic uncertainty, namely the error on the luminosity 
measurement. The latter is dominated by the 4\% systematic uncertainty 
on the determination of $\sigma_{\rm VOAND}$ which is due to uncertainties
of the beam intensities and in the analysis procedure of the van der Meer 
scan~\cite{SysV0AND}.

